Federated Linear Bandits with Finite Adversarial Actions

We study a federated linear bandits model, where $M$ clients communicate with a central server to solve a linear contextual bandits problem with finite adversarial action sets that may be different across clients. To address the unique challenges of adversarial finite action sets, we propose the FedSupLinUCB algorithm, which extends the principles of SupLinUCB and OFUL algorithms in linear contextual bandits. We prove that FedSupLinUCB achieves a total regret of $\tilde{O}(\sqrt{d T})$, where $T$ is the total number of arm pulls from all clients, and $d$ is the ambient dimension of the linear model. This matches the minimax lower bound and thus is order-optimal (up to polylog terms). We study both asynchronous and synchronous cases and show that the communication cost can be controlled as $O(d M^2 \log(d)\log(T))$ and $O(\sqrt{d^3 M^3} \log(d))$, respectively. The FedSupLinUCB design is further extended to two scenarios: (1) variance-adaptive, where a total regret of $\tilde{O} (\sqrt{d \sum \nolimits_{t=1}^{T} \sigma_t^2})$ can be achieved with $\sigma_t^2$ being the noise variance of round $t$; and (2) adversarial corruption, where a total regret of $\tilde{O}(\sqrt{dT} + d C_p)$ can be achieved with $C_p$ being the total corruption budget. Experiment results corroborate the theoretical analysis and demonstrate the effectiveness of FedSupLinUCB on both synthetic and real-world datasets.

==> macroset.tex <==
\usepackage{ifthen}
\usepackage{pgffor}

\ifthenelse{\equal{\dongningstyle}{true}}{
        \newcommand{\RVEC}[1]{\boldsymbol{\uppercase{#1}}}
        \newcommand{\RMAT}[1]{\underline{\boldsymbol{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\uppercase{#1}}
        \newcommand{\VEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\MAT}[1]{\boldsymbol{\underline{\lowercase{#1}}}}
}{
        \newcommand{\RVEC}[1]{\boldsymbol{#1}}
        \newcommand{\RMAT}[1]{\boldsymbol{\mathrm{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\uppercase{#1}}
        \newcommand{\VEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\MAT}[1]{\boldsymbol{\underline{\lowercase{#1}}}}
}

\ifthenelse{\equal{\fordiscussion}{true}}{
        \newcommand{\NONUM}{ }
}{
        \newcommand{\NONUM}{\nonumber}
}

\foreach \x in {A,...,Z}{%
         \expandafter\xdef\csname rv\x\endcsname{\noexpand\RVEC{\x}}
         \expandafter\xdef\csname rm\x\endcsname{\noexpand\RMAT{\x}}
         \expandafter\xdef\csname r\x\endcsname{\noexpand\RSCA{\x}}
         \expandafter\xdef\csname vv\x\endcsname{\noexpand\VEC{\x}}
         \expandafter\xdef\csname mm\x\endcsname{\noexpand\MAT{\x}}
}

\foreach \x in {a,...,z}{%
         \expandafter\xdef\csname rv\x\endcsname{\noexpand\RVEC{\x}}
         \expandafter\xdef\csname rm\x\endcsname{\noexpand\RMAT{\x}}
         %\expandafter\xdef\csname rr\x\endcsname{\noexpand\RSCA{\x}}
         \expandafter\xdef\csname vv\x\endcsname{\noexpand\VEC{\x}}
         \expandafter\xdef\csname mm\x\endcsname{\noexpand\MAT{\x}}
}



% IT or Communication Related
% Please define your \MII and \ENTH before including this file!
\newcommand{\snr}{\mathsf{snr}}
\newcommand{\mmse}[1]{\mathsf{mmse}\left( #1 \right)}
\newcommand{\inr}{\mathsf{INR}}
\newcommand{\MEXP}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\MEXPP}{\mathbb{E}}
\newcommand{\Prob}[1]{\mathsf{P}\left( #1 \right)}
\newcommand{\CProb}[2]{\mathsf{P}\left( \left.  #1 \right| #2 \right)}
\newcommand{\CProbR}[2]{\mathsf{P}\left(  #1 \left| #2 \right. \right)}
\newcommand{\Probb}{\mathsf{P}}
\newcommand{\LOG}[1]{\log \left( #1 \right)}
\newcommand{\MI}[1]{\ensuremath{\MII \left( #1 \right)}}
\newcommand{\CMI}[2]{\ensuremath{\MII \left(\left. #1 \right| #2 \right)}}
\newcommand{\CMIR}[2]{\ensuremath{\MII \left( #1 \left| #2 \right. \right)}}
\newcommand{\ENT}[1]{\ensuremath{\ENTH\left( #1 \right) }}
\newcommand{\CENT}[2]{\ensuremath{\ENTH\left( \left. #1 \right| #2 \right) }}
\newcommand{\CENTR}[2]{\ensuremath{\ENTH\left( #1 \left| #2 \right. \right) }}
\newcommand{\MARKOV}[3]{\ensuremath{#1\text{---}#2\text{---}#3}}
\newcommand{\IND}[1]{\mathbbm{1}_{\left( #1 \right)}}


% Other math notation
\newcommand{\uT}{\mathsf{T}}
\newcommand{\ud}{\mathsf{d}}
\newcommand{\trace}{\mathsf{tr}}
\newcommand{\HAT}[1]{\widehat{#1}}
\newcommand{\TIT}[1]{\widetilde{#1}}
\newcommand{\FLR}[1]{\lfloor #1 \rfloor}

% plain text related notations
\newcommand{\IE}{{\em i.e.}}
\newcommand{\EG}{{\em e.g.}}
\newcommand{\ETAL}{{\em et al.}}


% facilities
\newcommand{\fixme}[1]{{\color{Orangered} #1}}
\newcommand{\modify}[1]{{\color{Navyblue} #1}}


